Parallel Batch-dynamic Trees via Change Propagation

The dynamic trees problem is to maintain a forest subject to edge insertions and deletions while facilitating queries such as connectivity, path weights, and subtree weights. Dynamic trees are a fundamental building block of a large number of graph algorithms. Although traditionally studied in the single-update setting, dynamic algorithms capable of supporting batches of updates are increasingly relevant today due to the emergence of rapidly evolving dynamic datasets. Since processing updates on a single processor is often unrealistic for large batches of updates, designing parallel batch-dynamic algorithms that achieve provably low span is important for many applications. In this work, we design the first work-efficient parallel batch-dynamic algorithm for dynamic trees that is capable of supporting both path queries and subtree queries, as well as a variety of non-local queries. To achieve this, we propose a framework for algorithmically dynamizing static round-synchronous algorithms that allows us to obtain parallel batch-dynamic algorithms with good bounds on their work and span. In our framework, the algorithm designer can apply the technique to any suitably defined static algorithm. We then obtain theoretical guarantees for algorithms in our framework by defining the notion of a computation distance between two executions of the underlying algorithm. Our dynamic trees algorithm is obtained by applying our dynamization framework to the parallel tree contraction algorithm of Miller and Reif, and then performing a novel analysis of the computation distance of this algorithm under batch updates. We show that $k$ updates can be performed in $O(k \log(1+n/k))$ work in expectation, which matches an existing algorithm of Tseng et al. while providing support for a substantially larger number of queries and applications.

==> change-prop-proofs.tex <==
\section{Analysis of Change Propagation}

\subsubsection*{Proof of Theorem~\ref{thm:consistency}}

\begin{proof}
	
\end{proof}


\subsubsection*{Proof of Theorem~\ref{thm:round-based-propagation-bounds}}

\begin{proof}
	
\end{proof}

\subsubsection*{Proof of Theorem~\ref{thm:segment_tree_trace_distance}}

\begin{proof}
  
\end{proof}

\subsubsection*{Proof of Corollary~\ref{cor:segment_tree_fast}}

\begin{proof}

\end{proof}

\begin{todo}
  These proofs
\end{todo}

==> intro.tex <==
\section{Introduction}

A prominent feature of many modern large-scale computer systems is
their scale and the amount of data that they generate and process.
%
For example, Internet companies such as Facebook, Google, Microsoft,
and Twitter, among many others, periodically process and analyze huge
amounts of data.
%
Due to this rise in massive datasets, over the past decade there has
been significant interest in practical systems for processing such
``big data'', including MapReduce from Google~\cite{DeanGh08}, Dryad
from Microsoft~\cite{Isard+07}, Pregel~\cite{Malewicz+10},
GraphLab~\cite{Low+12}, and Dremel~\cite{Melnik+11}.
%
A widely accepted theoretical model for the MapReduce model of
computation, called Massively Parallel Computation Model or \MPC{}, has
also been
developed~\cite{ksv-mpc-2010,gsz-sorting-2011,anoy+geometric-2014} and
intensely studied in recent years to better understand how to design
large-scale distributed algorithms for massive datasets~\cite{
  IMS16,czumaj2018round, brandt2018matching, andoni2019log, ASW18,
  assadi2019sublinear,
  behnezhad2019exponentially,behnezhad2019massively}.
across
All of the theory and systems above are best suited for processing of \emph{static}, i.e., unchanging sets of data.
Motivated by the dynamic nature of large data sets, researchers and
practitioners  have more recently developed systems that can handle dynamic changes
to large data by performing as little work
as possible.
%
Such systems typically accept a \emph{batch} of changes, such as a
collection of edges to be inserted into a graph, and update the
property of interest, while striving to minimize total work and time.
%
Example systems include MapReduce Online~\cite{Condie+10}, Nectar
(extends DryadLINQ)~\cite{Gunda+10}, Incoop (extends Mapreduce and
Hadoop)~\cite{BhatotiaWiRoAcPa11}, Naiad~\cite{Murray+2013}, and
Google's proprietary system Percolator~\cite{PengDa10}.
%
Because these systems can all run on a parallel (shared memory)
machine and even on multiple machines, they make significant use
of parallelism to improve performance and achieve high throughputs.

Although researchers have shown significant practical improvements
in work and time by using these systems, their theoretical properties
are poorly understood.  In principle, it is possible to use classic
dynamic algorithms to process dynamic and large data sets, but this
would usually require breaking up changes into individual pieces and
applying them
sequentially~(e.g.,~\cite{chiangta92,ramalingamre93,demetrescufiit05-graphs,werneck08})
There has therefore been interest in designing theoretically efficient
parallel batch-dynamic
algorithms~\cite{simsiri2016work,tseng2018batch,acar2019parallel,italiano2019dynamic,durfee2019batch}.
The batch-dynamic setting extents classic dynamic algorithms to accept
batches of updates.  By applying batches it is often possible to get
significant parallelism.

In this paper, we observe that a relatively broad class of algorithms
are naturally amenable to dynamic parallelism.
We propose an \emph{algorithmic approach} to exploiting
dynamic parallelism exhibited by frequently changing data sets, as
well as handling batches of updates.
%
Our goal is not to devise a specific model that tries to capture the
details of the aforementioned practical systems or design new
batch-dynamic algorithms on an ad hoc basis but to develop an
algorithmic approach that can be applied more generally and uniformly
across a range of problems.
%
To this end, we propose a \emph{change-propagation} technique that can
be used to update the result of a parallel computation in response to
(batch of) changes to its input data.
%
\umut{And in this part here, this technique is so wonderful that it can actually be implemented in such a way to ``automatically'' transform parallel algorithms into dynamic parallel ones}
The technique is reasonably general and is applicable to any
\roundbased{} algorithm, i.e.,\ any parallel algorithm that operates in
a sequence of rounds.  \guy{Does it work for
  work for any algorithm that operates in a sequence of rounds?  I
  thought it had various limitations on number of reads, writes, etc.}
Each round executes in parallel across a set of processes.   Each
process starts by reading locations a shared
memory, then performs any computation in
isolation from the other processes and ends by writing back into
locations of the share memory, possibly different.
%
\Roundbased{} algorithms can be implemented in a variety of models,
including the \PRAM{} (work-depth) model and its variants, as well as
the \MPC{} model.
%
Likewise, change propagation accepts implementations in a variety of models and thus could be used to dynamize \roundbased{} algorithms.



The basic idea behind change propagation is to track dependencies
between global shared memory reads and local computations that depend
on them.
%
When the input is modified, change propagation ``pushes'' the change
through the computation by using the dependencies, in a round-by-round
fashion.
%
For example, if the input change affects (is consumed by) the local
computation performed by $p$ processes in round $1$, then the $p$
processes will repeat the affected work in parallel.
%
At the end of the round, the processes write their results to the
shared memory, which now constitutes a changes to ``tail'' of the
computation starting at round $2$, and thus can be handled in a
similar way.
%

We show that by paying some care to the precise representation of the
computation and the specifics of change propagation, the techniques
can be implemented efficiently, with nearly optimal overheads in
several broadly accepted models of parallel computation.  For example,
we show that on the classic \crcwpram{} model, change propagation can
be implemented with $O(1)$ work overhead, and only $O(\log^*(n))$
depth overhead, where $n$ is the number of parallel processes.
%
Furthermore, we develop a dependency-based cost model to bound the
cost of change propagation for specific \roundbased{} algorithms for
specific classes of changes.
%
The basic idea behind the cost model is to compute the ``distance''
between the computations before and after changes.
%
The cost model enables expressing and analyzing the cost of a dynamic
updates for a specific algorithm at a high level of abstraction and in
a uniform fashion across different algorithms.

Because change propagation applies to any \roundbased{} algorithm, it
can in principle be applied to a large class of parallel algorithms.
%
\guy{The following two sentences seem to repeat.}
As case studies, in this paper we consider three general algorithmic
problems, classic ``map-reduce'' style computations, computing
properties of dynamically changing sequences, and computing
properties of (possibly unbalanced) trees.
%
We show that three classic static parallel algorithmic techniques,
map reduce, list contraction, and tree contraction, can, under change
propagation, respond to changes efficiently in terms of both their work and depth.
%
Specifically, for list contraction and tree contraction, we show that dynamic
updates can be performed with work bounds that match the best known
hand-crafted data structures for the same problems, namely the
parallel batch-dynamic sequence structure and parallel batch-dynamic
trees structure from Tseng et al.~\cite{tseng2018batch}.
%
Furthermore, because they are applicable to all algorithms that can be expressed in terms of tree contraction, our results apply to a wider range of tree computations involving both subtree-based and path-based properties.
%

Our results are obtained by adapting the simple parallel algorithms
for these problems to the \roundbased{} setting, and performing a
novel analysis of the ``distance" of these algorithms, which may be of
independent interest.


%\umut{Add a paragraph here.}
Our proposed dynamization technique is algorithmic in the sense that it can be applied to any round-synchronous algorithm.
%
%This naturally raises the question of whether the technique can be applied fully automatically in practice.
%
%What we mean by this is whether it would be possible to take a parallel implementation of a round-synchronous algorithm and make it dynamic (and parallel) automatically.
%
%In this paper, we show that this is indeed possible by outlining a system for doing so.
%
%This system called \enginedelta{} (Delta Propogation Engine) provides the programmer with several primitives for implementing the algorithms in such a way that the implementations may be directly ``compiled into'' dynamic parallel algorithms.
%
%Specifically, algorithms implemented in \enginedelta{} can be executed on some input ``from scratch'' to generate some output, and then may be fed a change in the form of a ``delta'' that describes how the input should be modified (e.g., delete these set of edges and insert this other set of edges) and asked to update the output via change propagation.
%
...

%\umut{Added additional items on implementation}

The main contributions of this paper are:
\begin{itemize}
    \item An algorithmic framework for dynamizing \roundbased{} parallel algorithms,
    and a cost model for analysing the performance of such algorithmically dynamized algorithms
    \item The analysis of a dynamized tree contraction algorithm, which results in a data structure that matches
    the best known parallel dynamic tree data structure's work bounds while supporting both path and subtree queries.
\end{itemize}

\guy{summary of asymptotic costs, perhaps in a table or bulleted list.}

\guy{no mention of the initial run although it is a significant part
  of the body of the paper.   I guess we could remove from the body.}

%% \section{Introduction}

%% Due to the widespread availability of multicore machines and massively
%% parallel distributed systems, there has been significant recent
%% interest in designing \emph{parallel dynamic algorithms} that can
%% better make use of these resources for processing
%% dynamic updates and queries~\cite{acar2017brief, tseng2018batch,
%% acar2019parallel,italiano2019dynamic}. Since the traditional setting for dynamic algorithm
%% proceesses a single update or query at a time is and in some sense
%% inherently sequential, most of these works have considered
%% \emph{parallel batch-dynamic algorithms}, which process batches of
%% updates and queries.

%% In this paper we study a fundamental problem of automatically deriving
%% parallel batch-dynamic algorithms from efficient static parallel
%% algorithms. We describe a framework for generating parallel
%% batch-dynamic algorithms from static ones using a \emph{change
%% propagation} technique. Change propagation~\cite{acar2002adaptive} is
%% a method for automatically updating the output of an algorithm in
%% response to changes in its input. In SODA'04, Acar et al.\
%% \cite{acar2004dynamizing} described a machine model for automatically
%% dynamizing static sequential algorithms via a change propagation
%% method, and showed an analysis technique based on trace stability for
%% obtaining theoretical worst-case bounds on update performance.

%% Change propagation, and more broadly \emph{self-adjusting computation}
%% is motivated by the fact that writing correct and efficient dynamic
%% algorithms is already quite a non-trivial task. Due to issues
%% regarding concurrency, data consistency, and synchronization, writing
%% parallel dynamic algorithms by hand is even more challenging.
%% Therefore it is of both theoretical and practical interest to
%% understand how to automatically derive efficient parallel
%% batch-dynamic algorithms from static parallel algorithms.

%% Today, there are still a large numbers of parallel models that are
%% actively researched with different, often incomparable resource
%% measures, including the \PRAM{} (work-depth model), \MPC{} model, and
%% $\mathsf{CONGEST}$ model, just to name several.
%% In this paper, instead of restricting
%% our attention to a particular parallel model, we propose a simple framework
%% that is implementable on a variety of models, and define the notion
%% of a dynamic update and its cost, which translate into concrete
%% bounds in specific models.

%% Specifically, in this framework, we consider \emph{round-parallel} algorithms,
%% which are algorithms that perform parallel computations over
%% synchronous rounds. We define the notion of a \emph{computation distance},
%% which measures how much a computation differs when given one
%% input or another, and use this to analyse algorithms in this framework.
%% We then show how to obtain concrete bounds in various models for the algorithms
%% that we implement, in terms of their computation distance.

%% The main contributions of this paper are:
%% \begin{itemize}
%%     \item An automatic system for ...
%% \end{itemize}
%% \begin{todo}
%% Note  that  if  there  is  enough  stuff  we  want  to  state here, we can fork this into a results sub-section and state the main theorems here directly
%% \end{todo}


%% % Writing correct and efficient dynamic parallel algorithms is a nontrivial task.
%% % motivate dynamic algorithms. dynamic well studied in sequential setting.
%% % but not in parallel setting.
%% % one problem with the parallel setting is the model of computation.  There has not been a broad agreement.  earlier work assumed PRAM but this turned out to be not so practical.  Bridging models have been proposed (valiant).  Still, there is no broad concensus on what the model should be.
%% % %
%% % This presents a challenge.  Dynamic algorithms are complex. What should the assumptions be?
%% % We propose a structured approach.
%% % %
%% % We assume that the algorithm posseses a structure but don't make assumptions about the machine model.
%% % %
%% % We give ``distance'' based analysis that is model independent.
%% % %
%% % We can say for $k$ changes the distance is $O(...)$.
%% % Given this distance, we present an ``adaptation technique'' that can perform dynamic updates algorithmically by using the computation graphs themselves and without understanding the algorithms that generated the computation graphs.  This means that the adaptation techniques are generic on the algorithm that is being made dynamic.
%% %
%% %The adaptation techniques can in turn be implemented on a number of models, including on the traditional PRAM model as well as a threading model that  corresponds more closely to multithreaded and parallel languages being used today.






%% %In this paper, we describe a framework for generating dynamic parallel
%% %algorithms from static ones using a \emph{change propagation} technique. Change
%% %propagation \cite{acar2002adaptive} is a method for automatically updating the
%% %output of an algorithm in response to changes in its input. In SODA 2004, Acar
%% %et al.\ \cite{acar2004dynamizing} described a machine model for automatically
%% %dynamizing static sequential algorithms via a change propagation method, and showed
%% %an analysis technique based on trace stability for obtaining theoretical worst-case bounds
%% %on update performance.

%% \input{techniques}
%% \input{relwork}



%\guy{Seems like standard sequential dynamic algorithms should be
%  mentioned with an explanation of why they are inadequate.
%  Especially since we say that changes ``slowly'' over time.    Also
%  the reader who works on dynamic algorithms could be very annoyed.}
%\guy{Also it seems not to mention previous sequential work on
%  change propagation.    I
%  realize some of this is in related work, but if it motivates this
%  work it should be here.}



%has
%emerged~\cite{tseng2018batch, acar2019parallel}.
%In such a social graph, when a new edge emerges, it can be important
%to analyze  its impact and, for example, detect a connection between
%two vertices that were previously unreachable from each other.
%%
%Although, a static reachability algorithm could be executed after
%every change to  a graph, this approach wastes work and thus energy
%and could require at least linear  time.
%%
%As an other example, tables of transactions at a bank, or the
%web-pages on the internet both change daily, sometimes at a rapid
%rate, but in the changes are usually small relative to the overall
%size of the dataset.
%%
%Updating analyses over this data in time sub-linear in the size of the
%overall data may be critical to performing competitively in the
%market.
%Even though the changes to large data sets, such as bank transactions,
%or web-page updates on the internet are frequent and small,
%understanding their impact can be important.

